TimePoint: Accelerated Time Series Alignment via Self-Supervised Keypoint and Descriptor Learning

Fast and scalable alignment of time series is a fundamental challenge in many domains. The standard solution, Dynamic Time Warping (DTW), struggles with poor scalability and sensitivity to noise. We introduce TimePoint, a self-supervised method that dramatically accelerates DTW-based alignment while typically improving alignment accuracy by learning keypoints and descriptors from synthetic data. Inspired by 2D keypoint detection but carefully adapted to the unique challenges of 1D signals, TimePoint leverages efficient 1D diffeomorphisms, which effectively model nonlinear time warping, to generate realistic training data. This approach, along with fully convolutional and wavelet convolutional architectures, enables the extraction of informative keypoints and descriptors. Applying DTW to these sparse representations yield major speedups and typically higher alignment accuracy than standard DTW applied to the full signals. TimePoint demonstrates strong generalization to real-world time series when trained solely on synthetic data, and further improves with fine-tuning on real data. Extensive experiments demonstrate that TimePoint consistently achieves faster and more accurate alignments than standard DTW, making it a scalable solution for time-series analysis. Our code is available at https://github.com/BGU-CS-VIL/TimePoint

==> fig_arch.tex <==
\begin{figure*}[t]
\centering
\begin{tikzpicture}[
    font=\small,
    >=latex,
    line join=round,
    line cap=round,
    rounded corners,
    thick
]

%--------------------------------------------------------
% STYLES (adjust colors, sizes, etc.)
%--------------------------------------------------------
\tikzstyle{block} = [
    draw,
    minimum width=2.0cm,
    minimum height=0.8cm,
    align=center
]
\tikzstyle{encoderBlock}    = [block, fill=blue!20]
\tikzstyle{keypointDecoder} = [block, fill=green!20]
\tikzstyle{descDecoder}     = [block, fill=orange!25]
\tikzstyle{placeholderImg}  = [
    draw,
    fill=gray!10,
    minimum width=2.2cm,
    minimum height=1.0cm,
    align=center
]

%--------------------------------------------------------
% 1) INPUT A, ENCODER A, KEYPOINT DECODER A, DESCRIPTOR DECODER A (above)
%--------------------------------------------------------

% Input A
\node[
    label={[align=center]above:{\textbf{Input A}}}] 
    (inputA) 
    at (0,0)
    %[left, down, right, up]  
    {\includegraphics[trim=30mm 10mm 30mm 10mm, clip, width=0.25\linewidth]{figures/x1_pairwise_main_fig.png}};

% Encoder A (aligned horizontally with inputA)
\node[encoderBlock,
    right=1.4cm of inputA]
    (encA) 
    {WTConvEncoder};

% Keypoint Decoder A (aligned horizontally with encA)
\node[keypointDecoder, 
    right=1.4cm of encA] 
    (kpA) 
    {Keypoint\\Decoder};

% Descriptor Decoder A (above Keypoint Decoder A)
\node[descDecoder,
    above=1.4cm of kpA]
    (descA)
    {Descriptor\\Decoder};

% Connections for A
\draw[->] (inputA.east) -- (encA.west);
\draw[->] (encA.east) -- (kpA.west);

% From encoder A up to descriptor decoder A
\draw[->] (encA.north) -- ++(0,0.4) -| (descA.west);

%--------------------------------------------------------
% 2) INPUT B, ENCODER B, KEYPOINT DECODER B, DESCRIPTOR DECODER B (below)
%--------------------------------------------------------

% Input B
\node[
    label={[align=center]below:{\textbf{Input B}}},
    below=1.1cm of inputA]
    (inputB)
    {\includegraphics[trim=30mm 10mm 30mm 10mm, clip, width=0.25\linewidth]{figures/x2_pairwise_main_fig.png}};

% Encoder B (aligned horizontally with inputB)
\node[encoderBlock,
    right=1.4cm of inputB]
    (encB)
    {WTConvEncoder};

% Keypoint Decoder B (aligned horizontally with encB)
\node[keypointDecoder,
    right=1.4cm of encB]
    (kpB)
    {Keypoint\\Decoder};

% Descriptor Decoder B (below Keypoint Decoder B)
\node[descDecoder,
    below=1.4cm of kpB]
    (descB)
    {Descriptor\\Decoder};

% Connections for B
\draw[->] (inputB.east) -- (encB.west);
\draw[->] (encB.east) -- (kpB.west);

% From encoder B down to descriptor decoder B
\draw[->] (encB.south) -- ++(0,-0.4) -| (descB.west);

%--------------------------------------------------------
% 3) OUTPUT PLACEHOLDERS (in order top -> bottom)
%    1) descriptors_A
%    2) keypoints_A
%    3) keypoints_B
%    4) descriptors_B
%--------------------------------------------------------

% Descriptors A
\node[placeholderImg,
    right=3.2cm of descA]
    (descAOut)
    {Descriptors A};

% Descriptors B
\node[placeholderImg,
    right=3.2cm of descB]
    (descBOut)
    {Descriptors B};
% Time warping and Keypoint figure
\node[
    below=1.1cm of descAOut,
    %above=1.2cm of descBOut,
    align=center
] (pairwiseMainFig)
{   
    %[left, down, right, up]  
    \includegraphics[trim=5mm 5mm 5mm 5mm, clip, width=5cm]{figures/pairwise_main_fig.png}
};
\node[above=0.1cm of pairwiseMainFig, 
    align=center]
    (DTW_text)
    {DTW Keypoints Matching};

% Connect decoders to outputs
\draw[->] (descA.east) -- (descAOut.west);
\draw[->] (kpA.east)  -- (pairwiseMainFig.west);
\draw[->] (kpB.east)  -- (pairwiseMainFig.west);
\draw[->] (descB.east) -- (descBOut.west);

\end{tikzpicture}
\caption{High-level overview of the \textit{TimePoint} architecture. 
Each encoder (A or B) feeds into a Keypoint Decoder aligned horizontally, and a Descriptor Decoder positioned above (for A) or below (for B) the Keypoint Decoder. The final outputs (top to bottom) are Descriptors A, Keypoints A, Keypoints B, and Descriptors B. Dashed lines illustrate DTW warping between the Keypoints of A and B.}
\label{fig:temporalpoint-architecture}
\end{figure*}

==> fig_memory_consumption.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/MemoryConsumption.pdf}
    \caption{Total Memory Consumption (GB) for KNN computation on the GPU.}
\end{figure}

==> fig_robustness.tex <==
\begin{figure}
    \centering
    %[left, down, right, up] 
    \includegraphics[trim=0mm 0mm 0mm 10mm, clip, width=0.75\linewidth]{figures/robustness.pdf}
    \caption{\RED{Waiting for results}}
    \label{fig:robust}
\end{figure}

==> fig_supmat_dtw_path.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.49\linewidth]{./figures_supmat/BeetleFly_idx_0.png}
    \includegraphics[width=0.49\linewidth]{./figures_supmat/BeetleFly_idx_1.png}
    \caption{TimePoint Interest Point for the \texttt{BeetleFly} dataset}
    \label{fig:supmat:desc:kp:1}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=0.49\linewidth]{./figures_supmat/Phoneme_idx_0.png}
    \includegraphics[width=0.49\linewidth]{./figures_supmat/Phoneme_idx_2.png}
    \caption{TimePoint Interest Point for the \texttt{Phoneme} dataset}
    \label{fig:supmat:desc:kp2}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=0.49\linewidth]{./figures_supmat/Coffee_idx_4.png}
    \includegraphics[width=0.49\linewidth]{./figures_supmat/Coffee_idx_6.png}
    \caption{TimePoint Interest Point for the \texttt{Phoneme} dataset}
    \label{fig:supmat:desc:kp3}
\end{figure}

==> macros.tex <==
 %--------------------------------------------
% Add a period to the end of an abbreviation unless there's one
% already, then \xspace.
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
% \def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} \def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} 
% \def\wrt{with respect to }  % The extra space at the end means \wrt blah would 
% not end up as ``with respect toblah''. 
 
\def\dof{d.o.f\onedot}
% \def\etal{\emph{et al}\onedot}
\def\etal{\emph{et al}\onedot}
% \def\etal{\emph{et al}\onedot}
%
\def\iid{\emph{i.i.d}\onedot}
% \def\pdf{\emph{p.d.f}\onedot}



\makeatother
%--------------------------------------------------

\newcommand{\FIG}{Fig.~}
\newcommand{\FIGS}{Figs.~}
\newcommand{\EQN}{Eq.~}
% \newcommand{\EQN}{Equation }
\newcommand{\EQNS}{Eqs.~}
% \newcommand{\EQNS}{Equations }

%\newcommand{\SEC}{Sec.~}.  Use \autoref or ~\autoref instead.



% integers
\newcommand{\ZZ}{\ensuremath{\mathbb{Z}}}
\newcommand{\RR}{\ensuremath{\mathbb{R}}}
\newcommand{\Rtwo}{\ensuremath{\RR^2}}
\newcommand{\Rthree}{\ensuremath{\RR^3}}
\newcommand{\Rfive}{\ensuremath{\RR^5}}

\newcommand{\Rsix}{\ensuremath{\RR^6}}

\newcommand{\Rn}{\ensuremath{\RR^n}}
\newcommand{\Rd}{\ensuremath{\RR^d}}
\newcommand{\Rk}{\ensuremath{\RR^k}}
\newcommand{\Rm}{\ensuremath{\RR^m}}


% 
%positive integers
\newcommand{\Zplus}{\ensuremath{\ZZ^+}}
%positive reals
\newcommand{\Rplus}{\ensuremath{\RR^+}}


% set notation
% \newcommand{\set}[1]{\ensuremath{{\left\{#1\right\}}}}
\newcommand{\set}[1]{\ensuremath{{\{#1\}}}}
\newcommand{\tuple}[1]{\ensuremath{{(#1)}}}
\newcommand{\tupleLarge}[1]{\ensuremath{{\left(#1\right)}}}
\newcommand{\argmin}[1]{\ensuremath{\operatorname*{arg\,min}_{#1}}}
\newcommand{\argmax}[1]{\ensuremath{\operatorname*{arg\,max}_{#1}}}



\newcommand{\InnerProduct}[2]{\left\langle #1,#2 \right\rangle}

\newcommand{\norm}[1]{{{\left\|#1\right\|}}}
\newcommand{\sign}[1]{{\mathrm{sign}\left(#1\right)}}

\newcommand{\ellTwo}{\ell_2}
\newcommand{\ellTwoNorm}[1]{\norm{#1}_{\ellTwo}}
\newcommand{\ellOne}{\ell_1}




\newcommand{\MATRIX}[2][cccccccccccccccccccc]{\left[
 \begin{array}{#1}
 #2
 \end{array}
\right]}

\newcommand{\Mod}[1]{\ (\mathrm{mod}\ #1)}



% homogeneous coordinates
\newcommand{\bxh}{\widetilde{\bx}}

\newcommand{\RED}[1]{{{\color{red}{#1}}}}  
\newcommand{\BLUE}[1]{{{\color{blue}{#1}}}}
\newcommand{\GREEN}[1]{{{\color{green}{#1}}}}
\newcommand{\MAGENTA}[1]{{{\color{magenta}{#1}}}}  



\newcommand{\FREIFELD}[1]{\textbf{\MAGENTA{[FREIFELD says: #1]}}}
% Make your own

\newcommand{\TBD}{\RED{[TBD]}}
\newcommand{\TODO}[1]{\RED{[TODO: #1]}}




% In python: print_iterable(['\\bmdefine\\b{0}'.format(x)+'{'+x+'}' for x in 
% string.ascii_letters])

\bmdefine\ba{a}
\bmdefine\bb{b}
\bmdefine\bc{c}
\bmdefine\bd{d}
\bmdefine\be{e}
% \bmdefine\bf{f}  # Clashes with a standard command
\bmdefine\boldf{f}
\bmdefine\bg{g}
\bmdefine\bh{h}
\bmdefine\bi{i}
\bmdefine\bj{j}
\bmdefine\bk{k}
\bmdefine\bl{l}
\bmdefine\bm{m}
\bmdefine\bn{n}
\bmdefine\bo{o}
\bmdefine\bp{p}
\bmdefine\bq{q}
\bmdefine\br{r}
\bmdefine\bs{s}
\bmdefine\bt{t}
\bmdefine\bu{u}
\bmdefine\bv{v}
\bmdefine\bw{w}
\bmdefine\bx{x}
\bmdefine\by{y}
\bmdefine\bz{z}
\bmdefine\bA{A}
\bmdefine\bB{B}
\bmdefine\bC{C}
\bmdefine\bD{D}
\bmdefine\bE{E}
\bmdefine\bF{F}
\bmdefine\bG{G}
\bmdefine\bH{H}
\bmdefine\bI{I}
\bmdefine\bJ{J}
\bmdefine\bK{K}
\bmdefine\bL{L}
\bmdefine\bM{M}
\bmdefine\bN{N}
\bmdefine\bO{O}
\bmdefine\bP{P}
\bmdefine\bQ{Q}
\bmdefine\bR{R}
\bmdefine\bS{S}
\bmdefine\bT{T}
\bmdefine\bU{U}
\bmdefine\bV{V}
\bmdefine\bW{W}
\bmdefine\bX{X}
\bmdefine\bY{Y}
\bmdefine\bZ{Z}


\bmdefine\balpha{\alpha}
\bmdefine\bbeta{\beta}
\bmdefine\bgamma{\gamma}

\bmdefine\bdelta{\delta}
\bmdefine\btheta{\theta}
\bmdefine\blambda{\lambda}
\bmdefine\bphi{\phi}
\bmdefine\bxi{\xi}
\bmdefine\bzeta{\zeta}
\bmdefine\boldeta{\eta}
\bmdefine\bpi{\pi}

\bmdefine\bmu{\mu}
\bmdefine\brho{\rho}
\bmdefine\bomega{\omega}
\bmdefine\bOmega{\Omega}
\bmdefine\bPi{\Pi}

\bmdefine\bvarepsilon{\varepsilon}

\bmdefine\bDelta{\Delta}

\bmdefine\bTheta{\Theta}

\bmdefine\bSigma{\Sigma}
\bmdefine\bPsi{\Psi}
\bmdefine\bLambda{\Lambda}



\bmdefine\bzero{0}
\bmdefine\bone{1}
\bmdefine\binfty{\infty}

 \newcommand{\indicator}{\mathbbm{1}}


% In python 
% print_iterable(['\\newcommand{\\'+'{0}cal'.format(x)+'}{\\mathcal{'+x+'}}' 
% for x in string.ascii_uppercase])
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}


==> tables/tab_knn_results.tex <==
\begin{table}[t]
\caption{Number of \textbf{TimePoint} (TP) wins with different keypoint ratios compared to competing methods
on the UCR archive over \RED{101} datasets.}
\label{tab:ucr-wins}
%\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\scriptsize
\begin{tabular}{lcccc}
\toprule
\textbf{Method / \%KP} & \textbf{10\%} & \textbf{20\%} & \textbf{50\%} & \textbf{100\%} \\
\midrule
Euclidean                      & 83 &  86 &  84 &  86 \\
DTW                            &  47 & 54 & 53 &  60 \\
SoftDTW ($\gamma=0.1$)         &  60 & 64 & 67 &  67 \\
ShapeDTW (raw)                 &  45 & 61 & 59 & 65 \\
DTW-GI                         &  45 & 55 & 52 & 62 \\
\RED{TP+SoftDTW CUDA?}                         &  \TBD & \TBD & \TBD & \TBD \\

\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}


==> tables/tab_methods_comparison.tex <==
\begin{table}[h]
\caption{Comparison of Methods}
\centering
\scriptsize
\setlength{\tabcolsep}{1.5pt} % Adjust column separation
\begin{tabular}{p{1.5cm} p{1cm} p{1.2cm} p{1.1cm} p{1.5cm}}
\hline
Method & Interest Points? & Descriptors? & Learning? & Complexity \\
\hline
TemporalPoint & Yes & Yes & Yes & $O(L_{kp}^2)$ \\
DTW & No & No & No & $O(L^2)$ \\
SoftDTW & No & No & Yes & $O(L^2)$ \\
ShapeDTW & No & Yes & No  & $O(L^2)$ \\
GI-DTW & No & No & No  & $O(L^2)$ \\
%DCTW & No & Implicit & Yes  & High \\
\hline
\end{tabular}
\label{tab:method_comparison}
\end{table}


==> tables/tab_results_old.tex <==
\begin{table*}[ht]
\centering
\tiny
\caption{Comparison of CPU/GPU-based time series alignment methods. 
All lengths are percentages of the original time series length. 
KNN columns correspond to using $k=1,3,5$ for classification. 
Runtime is reported in hours (average and total).}
%\label{tab:results}
\begin{tabular}{llc|ccc|cc|c|cc}
\toprule
\multirow{2}{*}{\textbf{CPU/GPU}} 
  & \multirow{2}{*}{\textbf{Method}} 
  & \multirow{2}{*}{\textbf{Length}} 
  & \multicolumn{3}{c}{\textbf{KNN Accuracy}} 
  & \multicolumn{2}{c}{\textbf{Runtime (hrs)}} 
  & \multirow{2}{*}{\textbf{RAM}} 
  & \multicolumn{2}{c}{\textbf{\# Datasets}} \\
\cmidrule(lr){4-6}\cmidrule(lr){7-8}\cmidrule(lr){10-11}
 &  &  & \textbf{k=1} & \textbf{k=3} & \textbf{k=5} & \textbf{Avg} & \textbf{Total} &  & \textbf{Done} & \textbf{Discarded} \\
\midrule
\multirow{7}{*}{\textbf{CPU}} 
 & Euclidean               & 100\% & 0.371 & 0.378 & 0.384 & ... & ... & ... & ... & ... \\
 & DTW                     & 100\% & ... & ... & ... & ... & ... & ... & ... & ... \\
 & DTW-GI                  & 100\% & ... & ... & ... & ... & ... & ... & ... & ... \\
 & SoftDTW($\gamma=0.1$)   & 100\% & ... & ... & ... & ... & ... & ... & ... & ... \\
 & SoftDTW($\gamma=1$)     & 100\% & ... & ... & ... & ... & ... & ... & ... & ... \\
 & SoftDTW($\gamma=10$)    & 100\% & ... & ... & ... & ... & ... & ... & ... & ... \\
 & ShapeDTW?               & 100\% & ... & ... & ... & ... & ... & ... & ... & ... \\
 & FastDTW?                & 100\% & ... & ... & ... & ... & ... & ... & ... & ... \\
\midrule
\multirow{21}{*}{\textbf{GPU}}
 & DTW                     & 100\% & 0.706 & 0.687 & 0.676 & 1.83 & 	192 & ... & ... & ... \\
 & SoftDTW($\gamma=0.1$)   & 100\% & 0.677 & 0.650 & 0.632 & 0.02 & 2.1 & ... & ... & ... \\
 & SoftDTW($\gamma=1$)     & 100\% & 0.671 & 0.645 & 0.628 & 0.02 & 1.98 & ... & ... & ... \\
 & SoftDTW($\gamma=10$)    & 100\% & 0.670 & 0.644 & 0.625 & 0.02 & 1.94 & ... & ... & ... \\
\cmidrule(lr){2-11}
 & \multirow{4}{*}{TP+DTW} 
    & 10\%                 & 0.707 & ... & ... &  0.01 & \textbf{0.71} & ... & ... & ... \\
 &  & 20\%                 & 0.721 & ... & ... & 0.03 & 2.88 & ... & ... & ... \\
 &  & 50\%                 & 0.710 & ... & ... & 0.19 & 19.59 & ... & ... & ... \\
 &  & 100\%                & \textbf{0.732} & ... & ...  & 1.13 & 118.2 & ... & ... & ... \\
\cmidrule(lr){2-11}
 & \multirow{4}{*}{TP+SoftDTW($\gamma=0.1$)}
   & 10\%                   & 0.659 & ... & ... & 0.01 & 0.65 & ... & ... & ... \\
 &  & 20\%                  & 0.662 & ... & ... & 0.01 & 0.70 & ... & ... & ... \\
 &  & 50\%                  & 0.689 & ... & ... & 0.01 & 1 & ... & ... & ... \\
 &  & 100\%                 & 0.720 & ... & ... & 0.02 & 2.17 & ... & ... & ... \\
\cmidrule(lr){2-11}
 & \multirow{4}{*}{TP+SoftDTW($\gamma=1$)}
   & 10\%                   & 0.654 & ... & ... & 0.01 & 	0.52 & ... & ... & ... \\
 &  & 20\%                  & 0.659 & ... & ... & 0.01 & 0.56 & ... & ... & ... \\
 &  & 50\%                  & 0.687 & ... & ... & 0.01 & 0.86 & ... & ... & ... \\
 &  & 100\%                 & 0.711 & ... & ... & 0.02 & 2.16 & ... & ... & ... \\
\cmidrule(lr){2-11}
 & \multirow{4}{*}{TP+SoftDTW($\gamma=10$)}
   & 10\%                   & 0.655 & ... & ... & 0.01 & 0.5 & ... & ... & ... \\
 &  & 20\%                  & 0.658 & ... & ... & 0.01 & 0.55 & ... & ... & ... \\
 &  & 50\%                  & 0.680 & ... & ... & 0.01 & 0.85 & ... & ... & ... \\
 &  & 100\%                 & 0.703 & ... & ... & 0.02 & 2.02 & ... & ... & ... \\
\bottomrule
\end{tabular}
\end{table*}


==> tables_supmat/datasets_memory_consumption_table.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Dataset} & \textbf{Train Size} & \textbf{Test Size} & \textbf{Signal Length} \\
\hline
ChlorineConcentration & 467 & 3,840 & 166 \\
Crop & 7,200 & 16,800 & 46 \\
ECG5000 & 500 & 4,500 & 140 \\
TwoPatterns & 1,000 & 4,000 & 128 \\
UWaveGestureLibraryX & 896 & 3,582 & 315 \\
Wafer & 1,000 & 6,164 & 152 \\
Yoga & 300 & 3,000 & 426 \\
\hline
\end{tabular}
\caption{Datasets train size, test size, and signal length for GPU RAM consumption experiment.}
\label{tab:dataset_characteristics}
\end{table}
